A simple presentation of the effective topos

We propose for the Effective Topos an alternative construction: a realisability framework composed of two levels of abstraction. This construction simplifies the proof that the Effective Topos is a topos (equipped with natural numbers), which is the main issue that this paper addresses. In this our work can be compared to Frey's monadic tripos-to-topos construction. However, no topos theory or even category theory is here required for the construction of the framework itself, which provides a semantics for higher-order type theories, supporting extensional equalities and the axiom of unique choice.

==> AllOmega.tex <==
\subsection{Removing the duality between $Prop$ and $\Omega$}

At high level, in this framework proposition are either of the form
$F \in Prop$ or of the form $u \in |El(\Omega)|$. We can go from one form to the
other by using $el_\Omega$ and $prop$.

If we want to have only one level of propositions we have to :

\begin{itemize}

\item Define internal operator on $|El(\Omega)|$. For example we write \\
$u \Rightarrow v \equiv el_\Omega(prop(u) \Rightarrow prop(v))$. The operators
correspond to the operators of the internal logic of the topos $C$.

\item Reformulate the theorems in part 2 with the internal logic of
$|El(\Omega)|$.

\end{itemize}

With this we have only one level of proposition, so the use of the framework
will be simpler to use.


==> AllStrict.tex <==
\subsection{Strict logic}

If $A$ is an effective set and $u \in |El(A)|$ then we can write
$(u : A) \equiv |u =_{El(A)} u|$ and if $F \in |El(A)| \rightarrow Prop$
we can write $\forall u : A, F  \equiv \forall u \in |El(A)|, (u : A)
\Rightarrow F$ and $\exists u : A, F \equiv \exists u \in |El(A)|,
(u : A) \wedge F$.

This version of the axiom of choice holds :

$\vDash \forall F \in |El(A)| \rightarrow Prop,
(\forall u, v : A, F(u) \Rightarrow |u =_{El(A)} u'| \Rightarrow F)
\Rightarrow \\ (\forall u, v : A, F(u) \Rightarrow F(u') \Rightarrow
|u =_{El(A)} u'|) \Rightarrow (\exists u : A, F(u)) \Rightarrow \\
((d(F) : A) \wedge F(d(F)))$

This notation make the use of this framework less verbose.

\begin{remark}

We can adapt this for dependent types by writing $(u : w)$ for $||u =_w u||$.
We just have to be careful when doing proofs : to introduce a quantifier on $w$
we have to prove that $|w =_{El(Eff(T))} w'|$.

\end{remark}


==> Dep.tex <==
\subsection{Dependent types}

\begin{definition}[Definition of $Eff(T)$]

If $T$ is a set, we write $Eff(T)$ the effective set defined by:

\begin{itemize}

\item $|Eff(T)| \equiv (T \rightarrow Prop) \times
(T \rightarrow Prop) \rightarrow Prop$

\item $|f =_{Eff(T)} g| \equiv \\ (\forall u, v \in T \rightarrow Prop,
f(u, v) \Rightarrow f(v, u)) \wedge \\
(\forall u_1, u_2, u_3 \in T \rightarrow Prop, f(u_1, u_2) \Rightarrow
f(u_2, u_3) \Rightarrow f(u_1, u_3)) \wedge \\
(\forall u, v \in T \rightarrow Prop, f(u, v) \Leftrightarrow g(u, v))$

\end{itemize}

\end{definition}

\begin{definition}[Definition of $T_{/f}$ and $||u =_w v||$]

If $T$ is a set then we write:

\begin{itemize}

\item For all $f \in |Eff(T)|, T_{/f} \equiv el_{Eff(T)}(f)$

\item For all $w \in |El(Eff(T))|$, $u, v \in T \rightarrow Prop$,
$||u =_w v|| \equiv \exists f \in |Eff(T)|, w(f) \wedge f(u, v)$

\end{itemize}

\end{definition}

\begin{theorem}[Properties of $Eff(T)$] If $T$ is a set:

\begin{itemize}

\item $ \vDash \forall w, w' \in |El(Eff(T))|, u, v \in T \rightarrow Prop, \\
|w =_{El(Eff(T))} w'| \Rightarrow ||u =_w v|| \Rightarrow ||u =_{w'} v||$


\item $\vDash \forall f, g \in
((T \rightarrow Prop) \times (T \rightarrow Prop)) \rightarrow Prop, \\
(\forall u, v \in T \rightarrow Prop, f(u, v) \Rightarrow f(v, u))
\Rightarrow \\ (\forall u_1, u2, u3 \in T \rightarrow Prop, f(u_1, u_2)
\Rightarrow f(u_2, u_3) \Rightarrow f(u_1, u_3)) \Rightarrow \\
(\forall u, v \in T \rightarrow Prop, f(u, v) \Leftrightarrow g(u, v))
\Rightarrow \\ |T_{/f} =_{El(Eff(T))} T_{/g}|$ 

\item $\vDash \forall w \in |El(Eff(T))|, \forall u_1, u_2, u_3 \in
T \rightarrow Prop, |w =_{El(Eff(T))} w| \Rightarrow ||u_1 =_w u_2||
\Rightarrow ||u_2 =_w u_3|| \Rightarrow ||u_1 =_w u_3||$
\end{itemize}

\item $\vDash \forall w \in |El(Eff(T))|, \forall u, v \in T \rightarrow Prop,
|w =_{El(Eff(T))} w'| \Rightarrow ||u =_w v|| \Rightarrow ||v =_w u||$

\item $\vDash \forall f \in
((T \rightarrow Prop) \times (T \rightarrow Prop)), \forall u, v \in T
\rightarrow Prop, \\ (\forall u_1, u_2 \in T \rightarrow Prop, f(u_1, u_2)
\rightarrow f(u_2, u_1)) \Rightarrow \\ (\forall u_1, u_2, u_3 \in T
\rightarrow Prop, f(u_1, u_2) \Rightarrow f(u_2, u_3) \Rightarrow
f(u_1, u_3)) \Rightarrow \\ f(u, v) \Rightarrow ||u =_{T_{/f}} v||$

\item $\vDash \forall w, w' \in |El(Eff(T))|,
|w =_{El(Eff(T))} w| \Rightarrow |w' =_{El(Eff(T))} w'| \Rightarrow \\
(\forall u, v \in T \rightarrow Prop, ||u =_w v|| \Leftrightarrow
||u =_{w'} v||) \Rightarrow |w =_{El(Eff(T))} w'|$

\end{theorem}

This integrates well with our framework because generally the proofs only
depends on the proof of symmetry and transitivity of the equality of the
effective sets.

Example: dependent product.

\begin{definition}[Definition of $\Pi A f$]

If $A$ an effective set and $f : A \rightarrow Eff(T)$ then we write
$\Pi A f$ the effective set defined by:

\begin{itemize}

\item $|\Pi A f| \equiv |El(A)| \rightarrow (T \rightarrow Prop)$

\item $|g =_{\Pi A f} h| \equiv \forall u, v \in |El(A)|,
|u =_{El(A)} v| \Rightarrow ||g(u) =_{f(u)} h(v)||$

\end{itemize}

\end{definition}

We can also do some kind of polymorphism by quantifying over $El(Eff(T))$.

The full integration of dependent types in our framework is beyond the scope of this article.


==> Sys.tex <==
\section{Formal system}

$$A, B \recdef 1 \mid A \times B \mid A \rightarrow B \mid \Omega \mid
\{ \alpha \in A \mid F \} \mid Nat$$

$$u, v \recdef \alpha \mid <> \mid p_1(u) \mid p_2(v) \mid <u, v> \mid app(u, v)
\mid \Lambda \alpha : A . u \mid el(F) \mid d(\alpha : A . F) \mid Z \mid S(u)$$

$$F, G \recdef \top \mid \bot \mid F \wedge G \mid F \Rightarrow G \mid
\forall \alpha : A . F \mid \exists \alpha : A . F \mid |u =_A v| \mid prop(u)$$


$$\begin{array}{c}

\infer{\Derieff 1}{} \quad \infer{\Derieff \Omega}{} \quad
\infer{\Derieff Nat}{} \quad
\infer{\Derieff {A \times B}}{\Derieff A \quad \Derieff B} \quad
\infer{\Derieff {A \rightarrow B}}{\Derieff A \quad \Derieff B} \\\\
\infer{\Derieff {\{\alpha \in A \mid F\}}}{\Derieff A \quad
\Deriprop {\alpha : A} F \quad \Deriproof {} {} {\forall \alpha : A, \forall
\alpha' : A . F \Rightarrow |\alpha =_A \alpha'| \Rightarrow \subst F \alpha
{\alpha'}}} \\\\

\infer{\Deriexpr {\Gamma} {<>} 1}{} \quad
\infer{\Deriexpr \Gamma {p_1(u)} A}{\Deriexpr \Gamma u {A \times B}} \quad
\infer{\Deriexpr \Gamma {p_2(u)} B}{\Deriexpr \Gamma u {A \times B}} \quad
\infer{\Deriexpr \Gamma {<u, v>} {A \times B}}{\Deriexpr \Gamma u A \quad
\Deriexpr \Gamma v B} \\\\
\infer{\Deriexpr \Gamma {app(u, v)} B}{\Deriexpr \Gamma u {A \rightarrow B}
\quad \Deriexpr \Gamma u A}
\infer{\Deriexpr \Gamma {\Lambda \alpha : A . u} {A \rightarrow B}}{
\Derieff A \quad \Deriexpr {\Gamma, \alpha : A} u B} \quad
\infer{\Deriexpr \Gamma {el(F)} \Omega}{\Deriprop \Gamma F} \\\\
\infer{\Deriexpr \Gamma {d(\alpha : A . F)} A}{\Derieff A \quad
\Deriprop {\Gamma, \alpha : A} F} \quad
\infer{\Deriexpr \Gamma u {\{\alpha \in A \mid F\}}}{\Deriexpr \Gamma u A \quad
\Derieff {\{ \alpha \in A \mid F\}}} \quad
\infer{\Deriexpr \Gamma u A}{\Deriexpr \Gamma u {\{ \alpha \in A \mid F\}}} \\\\
\infer{\Deriexpr \Gamma Z {Nat}}{} \quad
\infer{\Deriexpr \Gamma {S(u)} {Nat}}{\Deriexpr \Gamma u {Nat}}\\\\

\infer{\Deriprop \Gamma \top}{} \quad
\infer{\Deriprop \Gamma \bot}{} \quad
\infer{\Deriprop \Gamma {F \wedge G}}{\Deriprop \Gamma F \quad \Deriprop
\Gamma G} \quad
\infer{\Deriprop \Gamma {F \Rightarrow G}}{\Deriprop \Gamma F \quad \Deriprop
\Gamma G} \\\\
\infer{\Deriprop \Gamma {\forall \alpha : A, F}}{\Derieff A \quad
\Deriprop {\Gamma, \alpha : A} F} \quad
\infer{\Deriprop \Gamma {\exists \alpha : A, F}}{\Derieff A \quad
\Deriprop {\Gamma, \alpha : A} F} \\\\
\infer{\Deriprop \Gamma {prop(u)}}{\Deriexpr \Gamma u \Omega} \quad
\infer{\Deriprop \Gamma {|u =_A v|}}{\Deriexpr \Gamma u A \quad
\Deriexpr \Gamma v A}\\\\

\infer{\Deriproof \Gamma \Sigma \top}{}\quad
\infer{\Deriproof \Gamma \Sigma F}{\Deriproof \Gamma \Sigma \bot \quad
\Deriprop \Gamma F}\quad
\infer{\Deriproof \Gamma {\Sigma, F} F}{}\\\\
\infer{\Deriproof \Gamma \Sigma {F \wedge G}}
{\Deriproof \Gamma \Sigma F \quad \Deriproof \Gamma \Sigma G}\quad
\infer{\Deriproof \Gamma \Sigma F}{\Deriproof \Gamma \Sigma {F \wedge G}}\quad
\infer{\Deriproof \Gamma \Sigma G}{\Deriproof \Gamma \Sigma {F \wedge G}}\\\\
\infer{\Deriproof \Gamma \Sigma {F \Rightarrow G}}
{\Deriprop \Gamma F \quad \Deriproof \Gamma {\Sigma, F} G}\quad
\infer{\Deriproof \Gamma \Sigma G}
{\Deriproof \Gamma \Sigma {F \Rightarrow G} \quad
\Deriproof \Gamma \Sigma F}\\\\
\infer{\Deriproof \Gamma \Sigma {\forall \alpha : A . F}}
{\Derieff A \quad \Deriprop \Gamma \Sigma \quad
\Deriproof {\Gamma, \alpha : A} \Sigma F}\quad
\infer{\Deriproof \Gamma \Sigma {\subst F \alpha u}}
{\Deriproof \Gamma \Sigma {\forall \alpha : A, F} \quad
\Deriexpr \Gamma u A}\\\\
\infer{\Deriproof \Gamma \Sigma {\exists \alpha : A, F}}
{\Deriproof \Gamma \Sigma {\subst F \alpha u} \quad \Deriexpr \Gamma u A}\quad
\infer{\Deriproof \Gamma \Sigma G}{
\Deriproof \Gamma \Sigma {\exists \alpha : A . F} \quad
\Deriprop \Gamma G \quad \Deriproof {\Gamma, \alpha : A} {\Sigma, F} G}\\\\

\end{array}$$

$$\begin{array}{c}

\infer{\Deriproof \Gamma \Sigma {\forall \alpha : A, \forall \beta : A,
|\alpha =_A \beta| \Rightarrow |\beta =_A \alpha|}}{\Derieff A}\\\\\
\infer{\Deriproof \Gamma \Sigma {\forall \alpha : A, \forall \beta : A,
\forall \gamma : A, |\alpha =_A \beta| \Rightarrow |\beta = \gamma|
\Rightarrow |\alpha = \gamma|}}{\Derieff A}\\\\

\infer{\Deriproof \Gamma \Sigma {|<> =_1 <>|}}{}\quad
\infer{\Deriproof \Gamma \Sigma {\forall \alpha : 1, \forall \beta : 1,
|\alpha =_1 \alpha| \Rightarrow |\beta =_1 \beta| \Rightarrow
|\alpha =_1 \beta|}}{}\\\\

\infer{\Deriproof \Gamma \Sigma {\forall \gamma : A \times B,
|p_1(\gamma) =_A p_1(\gamma)| \Rightarrow |\gamma =_{A \times B} \gamma|}}
{\Derieff A \quad \Derieff B}\\\\
\infer{\Deriproof \Gamma \Sigma {\forall \gamma : A \times B,
\forall \gamma' : A \times B, |\gamma =_{A \times B} \gamma'| \Rightarrow
|p_1(\gamma) =_A p_1(\gamma')|}}{\Derieff A \quad \Derieff B}\\\\
\infer{\Deriproof \Gamma \Sigma {\forall \gamma : A \times B,
|p_2(\gamma) =_B p_2(\gamma)| \Rightarrow |\gamma =_{A \times B} \gamma|}}
{\Derieff A \quad \Derieff B}\\\\
\infer{\Deriproof \Gamma \Sigma {\forall \gamma : A \times B,
\forall \gamma' : A \times B, |\gamma =_{A \times B} \gamma'| \Rightarrow
|p_2(\gamma) =_B p_2(\gamma')|}}{\Derieff A \quad \Derieff B}\\\\
\infer{\Deriproof \Gamma \Sigma {\forall \alpha : A, \forall \beta : A,
|<\alpha, \beta> =_{A \times B} <\alpha, \beta>| \Rightarrow
(|\alpha =_A \alpha| \wedge |\beta =_B \beta|)}}
{\Derieff A \quad \Derieff B}\\\\
\infer{\Deriproof \Gamma \Sigma {\forall \alpha, \alpha' : A,
\forall \beta, \beta' : B, |\alpha =_A \alpha'| \Rightarrow
|\beta =_B \beta'| \Rightarrow |<\alpha, \beta> =_{A \times B}
<\alpha', \beta'>|}}{\Derieff A \quad \Derieff B}\\\\
\infer{\Deriproof \Gamma \Sigma {\forall \alpha : A, \forall \beta : B,
|\alpha =_A \alpha| \Rightarrow |\beta =_B \beta| \Rightarrow
|p_1(<\alpha, \beta>) =_A \alpha|}}{\Derieff A \quad \Derieff B}\\\\
\infer{\Deriproof \Gamma \Sigma {\forall \alpha : A, \forall \beta : B,
|\alpha =_A \alpha| \Rightarrow |\beta =_B \beta| \Rightarrow
|p_2(<\alpha, \beta>) =_B \beta|}}{\Derieff A \quad \Derieff B}\\\\
\infer{\Deriproof \Gamma \Sigma {\forall \gamma, \gamma' : A \times B,
|p_1(\gamma) =_A p_1(\gamma')| \Rightarrow |p_2(\gamma) =_B p_2(\gamma')|
\Rightarrow |\gamma =_{A \times B} \gamma'|}}{\Derieff A \quad \Derieff B}\\\\

\end{array}$$

